FPT: Improving Prompt Tuning Efficiency via Progressive Training

Recently, prompt tuning (PT) has gained increasing attention as a parameter-efficient way of tuning pre-trained language models (PLMs). Despite extensively reducing the number of tunable parameters and achieving satisfying performance, PT is training-inefficient due to its slow convergence. To improve PT's training efficiency, we first make some novel observations about the prompt transferability of "partial PLMs", which are defined by compressing a PLM in depth or width. We observe that the soft prompts learned by different partial PLMs of various sizes are similar in the parameter space, implying that these soft prompts could potentially be transferred among partial PLMs. Inspired by these observations, we propose Fast Prompt Tuning (FPT), which starts by conducting PT using a small-scale partial PLM, and then progressively expands its depth and width until the full-model size. After each expansion, we recycle the previously learned soft prompts as initialization for the enlarged partial PLM and then proceed PT. We demonstrate the feasibility of FPT on 5 tasks and show that FPT could save over 30% training computations while achieving comparable performance.

==> sections/4_related_work.tex <==
\section{Related Work}

\paragraph{Prompt Tuning.} Since the emergence of Pretrained Language Models \citep{devlin2018bert, liu2019roberta, xlnet2019}, PLM have achieved excellent performance on many natural language processing tasks relying on their powerful natural language understanding and generation capabilities. However, with the emergence of larger and larger PLMs like T5 \citep{2020t5} and GPT-3 \citep{gpt3}, the method of directly adjusting all the parameters of PLM requires huge storage and memory resources and is not flexible for these PLMs applied on massive downstream natural languge tasks. Therefore, parameter efficient tuning methods \citep{houlsby2019parameter, mahabadi2021compacter, hu2021lora} attract more and more attention, among which prompt tuning \citep{lester-etal-2021-power} is a simple and effective one. By prepending a few trainable embeddings before sequence, prompt tuning can acheive comparable performance with finetuning. With size of PLM getting larger, the performance of prompt tuning gets closer to finetuning even surpassing finetuning on T5$_{\texttt{XXL}}$, showing great potential to utilize more powerful PLMs in future. But due to the longer input length \citep{mahabadi2021compacter} and slow convergence speed \citep{su2021transferability}, its training efficiency is an important drawback of prompt tuning and may limit its practical application.

\paragraph{Progressive Training.} Progressive training has been used in pretraining process to improve training efficiency \citep{pmlr-v97-gong19a} since pretraining usually needs much computation resource. They started training with a shallow model and the depth of model grow deeper along the training process by stacking layers of the trained shallow model. In this way, the pretraining efficiency can be improved a lot. To further improve training efficiency, \citet{chen2021bert2bert} propose some initialization methods to keep function preserved and better reuse parameters of shallow models when increase the size of training model. Different from their methods, we apply the progressive training process into prompt tuning, which doesn't need to modify parameters of models but only an additional soft prompts. Therefore, instead of stacking layers of current model, we need to select the informative parameters of the whole PLM and check the transferability of soft prompts between selected partial models. And besides of modifying the depth of model, we also propose to modify hidden dimensions of model to further improve training efficiency.

